Incentive Compatibility in the Auto-bidding World

Auto-bidding has recently become a popular feature in ad auctions. This feature enables advertisers to simply provide high-level constraints and goals to an automated agent, which optimizes their auction bids on their behalf. In this paper, we examine the effect of different auctions on the incentives of advertisers to report their constraints to the auto-bidder intermediaries. More precisely, we study whether canonical auctions such as first price auction (FPA) and second price auction (SPA) are auto-bidding incentive compatible (AIC): whether an advertiser can gain by misreporting their constraints to the autobidder. We consider value-maximizing advertisers in two important settings: when they have a budget constraint and when they have a target cost-per-acquisition constraint. The main result of our work is that for both settings, FPA and SPA are not AIC. This contrasts with FPA being AIC when auto-bidders are constrained to bid using a (sub-optimal) uniform bidding policy. We further extend our main result and show that any (possibly randomized) auction that is truthful (in the classic profit-maximizing sense), scalar invariant and symmetric is not AIC. Finally, to complement our findings, we provide sufficient market conditions for FPA and SPA to become AIC for two advertisers. These conditions require advertisers' valuations to be well-aligned. This suggests that when the competition is intense for all queries, advertisers have less incentive to misreport their constraints. From a methodological standpoint, we develop a novel continuous model of queries. This model provides tractability to study equilibrium with auto-bidders, which contrasts with the standard discrete query model, which is known to be hard. Through the analysis of this model, we uncover a surprising result: in auto-bidding with two advertisers, FPA and SPA are auction equivalent.

==> SPA_discrete.tex <==


\subsection{Warm Up: Second Price Auction is not AIC!}
Let us start with a simple example of auto-bidding with the second-price auction. Through this example, we will demonstrate the process of determining the equilibrium in an auto-bidding scenario and emphasize a case where the advertiser has an incentive to misreport their budget.



Consider two budget-constrained advertisers and three queries $Q=\{q_1,q_2,q_3\}$, where the expected value of winning query $q$ for advertiser $a$ is denoted by $v_a(q)$, and it is publicly known (as in Table \ref{tab:budget-second price}). At first, each advertiser reports their budget to the auto-bidder (denoted by $B_1=2$, and $B_2=4$). Then we have auto-bidder agents, one for each advertiser. The auto-bidder agents submit a bidding profile (to maximize their advertisers' obtained value subject to the budget constraint). Next, there will be a second-price auction per query, i.e., after the auto-bidders bid on behalf of advertisers, each query is allocated according to a second-price auction. 
% \begin{table}[!htp]
%     \centering
%     \begin{tabular}{c|c|c|c}
%          & $q_1$& $q_2$& $q_3$ \\\hline
%         Advertiser 1 & 4 & 3 &2\\
%         Advertiser 2 & 1 & 1.3 &10\\
%     \end{tabular}
%     \caption{Budget Constraint Non-AIC Example: The value of each query for each advertiser.}
%     \label{tab:budget-second price}
% \end{table}


Next, we calculate the equilibrium between the auto-bidder agents. 
Since each auto-bidder agent's bidding profile change the cost of queries for the rest of the agents, each agent should choose a bidding profile that is the best response with respect to the other agents. Here, we use the result of \cite{Aggarwal19}\footnote{The result states that uniform bidding is \emph{almost} optimal. However, by applying their proof to our example with single-slot queries and loose constraints one can see that uniform bidding is actually optimal. We will formalize this later in Appendix~\ref{appendix: tcpa second price warm up}.}, which states that the best response strategy in any truthful auto-bidding auction is uniform bidding. In other words, each agent optimizes over one variable, a bidding multiplier $\mu_a$, and then bids on query $q$ with respect to the scaled value  $\mu_av_a(q)$. 

First, we claim that with budgets $B_1=2$ and $B_2=4$, an equilibrium exists such that advertiser 1 only wins $q_1$.
We claim that $\mu_1=.5$ and $\mu_2=1$ result in such an equilibrium. To this end, we need to check: 1) Allocation: advertiser 1 wins $q_1$, 2) 
Budget constraints are satisfied, and 3) Best response: The auto-bidder agents do not have the incentive to increase their multiplier. Therefore, these three conditions are checked next:
 \begin{enumerate}
    \item \emph{Allocation inequalities:} For each query, the advertiser with the highest bid wins it.
\[\frac{v_1(q_1)}{v_2(q_1)}\geq \frac{\mu_2}{\mu_1}=\frac{1}{.5}\geq \frac{v_1(q_2)}{v_2(q_2)}\geq \frac{v_1(q_3)}{v_2(q_3)}.\]
        \item
       \emph{ Budget constraints:} Since the auction is second-price the cost of query $q$ for advertiser 1 is $\mu_2v_2(q)$ and for for advertiser 1 is $\mu_1v_1(q)$). So, we must have the following inequalities to hold so that the budget constraints are satisfied:
    \[2=B_1\geq \mu_2 v_2(q_1)=1\qquad \text{(Advertiser 1)},\]
    \[4=B_2\geq \mu_1(v_1(3)+v_1(q_2))=2.5\qquad \text{(Advertiser 2)}.\]
\item \emph{Best response:} Does the advertiser's agent have incentive to higher their multiplier to get more queries? If not, they shouldn't afford  the next cheapest query.
    \[2<  \mu_2(v_2(q_1)+v_2(q_2))=2.3\qquad \text{(Advertiser 1)},\]
    \[4< \mu_1(v_1(q_3)+v_1(q_2)+v_1(q_1))=4.5\qquad \text{(Advertiser 2)}.\]
    \end{enumerate}
    Since all the three conditions are satisfied, we have found an equilibrium that advertiser 1 wins $q_1$ and advertiser 2 wins $q_2$ and $q_3$. 


Now, consider the scenario that advertiser 1 wants to strategically report their decision on their reported budget $B_1$. Intuitively, suppose the first advertiser decreases their budget. In that case, the budget constraint for the auto-bidder agent should be harder to satisfy, and hence the advertiser should not get a higher value. But, contrary to this intuition, this is not what always happens.  

Assume that advertiser 1 report a lower budget $B_1'=1$. Then we show that the equilibrium is unique and advertiser 1 always wins $q_1$ and $q_2$ (more queries than the initial case with a higher budget). First, we show $\mu_1'=\frac{1}{2.3}$, and $\mu_2'=1$ results in an equilibrium:
\begin{enumerate}
    \item Allocation: advertiser 1 wins $q_1$ and $q_2$ since it has a higher bid on them,
\[\frac{v_1(q_1)}{v_2(q_1)}\geq\frac{v_1(q_2)}{v_2(q_2)}\geq \frac{\mu'_2}{\mu'_1}=\frac{1}{2.3}\geq  \frac{v_1(q_3)}{v_2(q_3)}.\]
    \item Budget constraints:
    \[4\geq v_1(q_3),\qquad\text{and }\]
    \[1= (1/2.3)(v_2(q_1)+v_2(q_2)).\]
\item Best response: 
    \[4< 1(v_1(q_3)+v_1(q_2)),\qquad\text{and}\]
    \[1< (1/2.3) (v_2(q_1)+v_2(q_2)+v_2(q_3)).\]
\end{enumerate} 
So far, we have proved that an equilibrium exists where advertiser 1 can get two queries. 
    Next, we prove this equilibrium is unique. First, note that there's no equilibrium such that advertiser 1 wins all the queries. To see this, note that the multiplier of advertiser 1 is at most $1$. Hence, the price of $q_3$ for advertiser 2 is within their budget, and they have incentive to increase their multiplier to buy $q_3$. Similarly, one can see that in any equilibrium advertiser 1 gets at least $q_1$, since its highest price is within their budget.

    Now,    assume some equilibrium exists with bidding prices  $\tilde\mu_1$ and $\tilde\mu_2$  such that advertiser  1 gets only $q_1$. Then
\[ \frac{\tilde \mu_1(v_1(1)+v_1(2)+v_1(3))}{B_2}>1\geq  \frac{\tilde \mu_2v_2(1)}{B_1},\] 
where the first inequality is because advertiser 2's multiplier is the best-response, and the second is coming from the budget constraint for advertiser 1.
Therefore,
\[ \frac{B_1}{B_2}\frac{v_1(1)+v_1(2)+v_1(3)}{v_2(1)}\geq \frac{\tilde \mu_2}{\tilde \mu_1},\]
But $\frac{v_1(2)}{v_2(2)}\geq \frac{B_1}{B_2}\frac{v_1(1)+v_1(2)+v_1(3)}{v_2(1)}=\frac{9}{4}$, and thus $\frac{v_1(2)}{v_2(2)}>\frac{\tilde\mu_2}{\tilde\mu_1}$. This is in contradiction with allocation inequalities since advertiser 2 wins $q_2$. Therefore, we proved with $B_1=1$ and $B_2=4$ the equilibrium is unique such that advertiser 1 wins $q_1$ and $q_2$. 


% In fact, increasing the budget could change the set of equilibrium so that the advertiser end up getting worse allocations. As a result of increased budget, the current bids of the first advertiser are not necessarily best response, so the auto-bidder might increase their bids which would result in getting more queries. But now, the other advertiser who lost a query has to increase their bids as well. This will result in increased price that the first advertiser cannot afford anymore. As a result in a potential new equilibrium the first advertiser might bid lower while they have increased their budget, and the second advertiser will bid higher while their budget has not changed. \todo{}
This surprising example leads to the first main result of the paper as formalized in the following theorem.
In Appendix~\ref{appendix: tcpa second price warm up}, we will generalize the above example to the case of tCPA-constrained advertisers with the same set of queries in Table~\ref{tab:budget-second price}.
\begin{theorem}\label{thm: second price Warm up}
Auto-bidding with second price auction is not AIC, i.e., in some scenarios advertisers have incentive to report a stricter constraint to obtain a higher value.
This result holds as long as the advertisers are all either budget-constrained or tCPA constrained.
\end{theorem}
% \begin{proof}
% Consider two budget-constrained advertisers, and 3 queries $Q=\{q_1,q_2,q_3\}$. The value of each advertiser per query is specified in Table \ref{tab:budget-second price}. Initially, budgets of the  two advertisers are $B_1=1$ and $B_2=4$. In this case, we claim that there exists an equilibrium where the first advertiser gets both queries $q_1$ and $q_2$.  Then we show that if advertiser 1 increase their budget to $B_1'=2$, then the equilibrium is unique and in this equilibrium advertiser 1 only wins $q_1$.
% \begin{table}[!htp]
%     \centering
%     \begin{tabular}{c|c|c|c}
%          & $q_1$& $q_2$& $q_3$ \\\hline
%         Advertiser 1 & 4 & 3 &2\\
%         Advertiser 2 & 1 & 1.3 &10\\
%     \end{tabular}
%     \caption{Budget Constraint Non- AIC Example: The value of each query for each advertiser.}
%     \label{tab:budget-second price}
% \end{table}

% We start characterizing equilibrium when $B_1=1, B_2=4$. Given Theorem 1 by \cite{Aggarwal19}, we only need to find the bidding multipliers $\mu_1$ and $\mu_2$ for each advertiser. First, we claim that $\mu_1=1$ and $\mu_2=\frac{1}{2.3}$ results in an equilibrium such that advertiser 1 gets $q_1$ and $q_2$. To this end, we need to check: 1) Allocation: advertiser 1 wins $q_1$ and $q_2$, 2) 
% Budget constraints are satisfied, and 3) Best response: The auto-bidder agents do not have incentive to increase their multiplier. These three conditions are checked next:
% \begin{enumerate}
%     \item Allocation: advertiser 1 wins $q_1$ and $q_2$ since it has a higher bid on them
% \[\frac{v_1(1)}{v_2(1)}\geq\frac{v_1(2)}{v_2(2)}\geq \frac{\mu_2}{\mu_1}=\frac{1}{2.3}\geq  \frac{v_1(q_3)}{v_2(q_3)}.\]
%     \item Budget constraints are satisfied:
%     \[4\geq v_1(q_3),\qquad\text{and }\]
%     \[1= (1/2.3)(v_2(1)+v_2(2)).\]
% \item Best response: non of the advertiser have the budget to win more queries if they increase their multiplier. Since if they want to win a new query they have to pay at least as much as the other advertiser's bids.
%     \[4< 1(v_1(q_3)+v_1(q_2)),\qquad\text{and}\]
%     \[1< (1/2.3) (v_2(q_1)+v_2(q_2)+v_2(q_3)).\]
% \end{enumerate} 

% So far, we have proved that initially there exists an equilibrium where advertiser 1 can get two queries. 
%     Next, we prove this equilibrium is unique. First, note that there's no equilibrium such that advertiser 1 wins all the queries. To see this, note that the multiplier of advertiser 1 is at most $1$. Hence the price of $q_3$ for advertiser 2 is within their budget of 2, and they have incentive to increase their multiplier to buy $q_3$. Similarly, one can see that in any equilibrium advertiser 1 gets at least $q_1$, since its highest price is within their budget.

%     Now,    assume that there exists some equilibrium with bidding prices  $\tilde\mu_1$ and $\tilde\mu_2$  such that advertiser  1 gets only $q_1$. Then
% \[ \frac{\tilde \mu_1(v_1(1)+v_1(2)+v_1(3))}{B_2}>1\geq  \frac{\tilde \mu_2v_2(1)}{B_1},\] 
% where the first inequality is because advertiser 2's multiplier is the best-response, and the second inequality is coming from the budget constraint for advertiser 1.
% Therefore,
% \[ \frac{B_1}{B_2}\frac{v_1(1)+v_1(2)+v_1(3)}{v_2(1)}\geq \frac{\tilde \mu_2}{\tilde \mu_1},\]
% But $\frac{v_1(2)}{v_2(2)}\geq \frac{B_1}{B_2}\frac{v_1(1)+v_1(2)+v_1(3)}{v_2(1)}=\frac{9}{4}$, and thus $\frac{v_1(2)}{v_2(2)}>\frac{\tilde\mu_2}{\tilde\mu_1}$. This is in contradiction with allocation inequalities since advertiser 2 wins $q_2$. Therefore, we proved with $B_1=1$ and $B_2=4$ the equilibrium is unique such that advertiser 1 wins $q_1$ and $q_2$. 
    
%     Now, consider the case that advertiser 1 increases their budget to $B_1'=2$. We show that there exists an equilibrium in which advertiser 1 only gets $q_1$. Let $\mu_1'=.5$, $\mu'_2=1$. As before, we need to check three conditions:
%     \begin{enumerate}
%     \item Allocation inequalities:
% \[\frac{v_1(1)}{v_2(1)}\geq \frac{1}{.5}\geq \frac{v_1(2)}{v_2(2)}\geq \frac{v_1(3)}{v_2(3)}.\]
%         \item
%         Budget constraints:
%     \[2\geq v_2(1)\qquad \text{(Advertiser 1)},\]
%     \[4\geq .5(v_1(3)+v_1(2))\qquad \text{(Advertiser 2)}.\]
% \item Best response: 
%     \[2<  (v_2(1)+v_2(2))\qquad \text{(Advertiser 1)},\]
%     \[4< .5(v_1(3)+v_1(2)+v_1(1))\qquad \text{(Advertiser 2)}.\]
%     \end{enumerate}
    
%     Since all the conditions hold, we proved that advertiser 1 might end up with $q_1$ in an equilibrium, which is worse of what they can get with a lower budget.


% In Appendix~\ref{appendix: tcpa second price warm up}, we will show that there exists an example of two tCPA constrained advertisers with the same set of queries in Table~\ref{tab:budget-second price} such that the resulting equilibrium is not weakly AIC for tCPA constraints.
% \end{proof}

